Deterministic Extractors for Additive Sources

We propose a new model of a weakly random source that admits randomness extraction. Our model of additive sources includes such natural sources as uniform distributions on arithmetic progressions (APs), generalized arithmetic progressions (GAPs), and Bohr sets, each of which generalizes affine sources. We give an explicit extractor for additive sources with linear min-entropy over both $\mathbb{Z}_p$ and $\mathbb{Z}_p^n$, for large prime $p$, although our results over $\mathbb{Z}_p^n$ require that the source further satisfy a list-decodability condition. As a corollary, we obtain explicit extractors for APs, GAPs, and Bohr sources with linear min-entropy, although again our results over $\mathbb{Z}_p^n$ require the list-decodability condition. We further explore special cases of additive sources. We improve previous constructions of line sources (affine sources of dimension 1), requiring a field of size linear in $n$, rather than $\Omega(n^2)$ by Gabizon and Raz. This beats the non-explicit bound of $\Theta(n \log n)$ obtained by the probabilistic method. We then generalize this result to APs and GAPs.

==> extrff.tex <==
\section{Polynomial HAP sources}\label{sec:extrff}

\begin{comment}
\paragraph{Polynomial HAP sources as structured sources}


In this section, we work in the setting of polynomials over a finite field $\Fq$ with $q$ elements, where $q$ is a prime power. 
Let $Q \in \Fq[t]$ be monic irreducible and let $deg(Q)=n$. Then, $\Fq[t]/(Q)$ is isomorphic to $\Fq^n$. That is, every element of the field $\Fq^n$ can be thought of as a polynomial mod $Q$. We shall stick with the polynomial way of representing the field. Let $R(t) \in \Fq[t]$. Then consider the ideal $I=\{R(t)P(t):P \in \Fq[t]\}$. We note that $\Fq[t]$ is a principal ideal domain and hence every ideal is of this form. Now, instead of running over all polynomials, let us only consider low degree polynomials, say up to degree $d$. We want to see what $d$ allows extraction from such sources. Thus, a subideal source in a field $\Fq[t]/(Q)$ corresponding to $R(t)$ is defined as $X=\{RP \pmod Q : deg P \leq d\}$. Note that this is a special case of an affine source. 

It is easy to observe that such a source has very low doubling ($|X+X| \leq 2|X|$) and very large symsets ($|Sym_1(X)|\geq |X|$) and hence is clearly a structured source. However, we shall see that we can do much better than using the extractor for general structured sources. Our main theorem on extractors will follow from the main technical lemma on a short character sum on $\Fq[t]$ over monic degree $d$ polynomials modulo $Q$ but can be easily extended to all degree at most $d$ polynomials. First, we can easily extend this to get a bound over all degree (exactly) $d$ polynomials. Now to allow for at most degree $d$ polynomials, we run the same bound on $d-1$ polynomials and so on until say $d/2$ beyond which we apply a trivial $q^{d/2}$ bound without losing much in the total error. The multiplication by $R(t)$ is permitted because the character is multiplicative.

This also gives a way to extract from sources that can be encoded as polynomials and then the rich structure of polynomials can be put to good use. For example, suppose a source has a few consecutive bits of pure randomness (say $a_0,\cdots a_{r-1}$) and it places them at starting locations $i_1, i_2 \cdots i_k$ (say). Then, we consider the polynomial hidden in different chunks in $\Fq^n$. That is say the source looks like $r\ldots r$ for some randomness $r$. The theorem states that even if $r$ is logarithmic in $n$ for even constant field size, one can extract from such a source by viewing $r$ as the coefficients of $P$ and $R(t)=1+t^c$ form some large $c$ and considering the corresponding subideal source. 
\end{comment}


In this section, we work in the setting of polynomials over a finite field $\Fq$ with $q$ elements, where $q$ is a prime power. 
Let $Q \in \Fq[t]$ be monic irreducible and let $\deg(Q)=n$. Then, $\Fq[t]/(Q)$ is isomorphic to $\Fq^n$. That is, every element of the field $\Fq^n$ can be thought of as a polynomial mod $Q$. We shall stick with the polynomial way of representing the field. Let $R(t) \in \Fq[t]$. Then the set $I=\{R(t)P(t)\pmod Q:|P| \leq s\}$ forms a homogenous arithmetic progression over polynomials. Here $R(t)$ is the \textit{common difference} and it can be seen that this is analogous to $\{id:i \leq k\}$ over the integers. Here, $|P|$ denotes the norm of the polynomial $P$ which is defined as $q^{\deg(P)}$. This is usually referred to as an HAP in function fields. We want to allow extraction from as small a source as possible. 

It is easy to observe that such a source has very low doubling ($|X+X| \leq |X|$) and very large symsets ($|Sym_1(X)|\geq |X|$) and hence is clearly a structured source. However, we shall see that we can do much better than using the extractor for general structured sources. Our main theorem on extractors will follow from the main technical lemma on a short character sum on $\Fq[t]$ over monic degree $d$ polynomials modulo $Q$ but can be easily extended to all degree at most $d$ polynomials. First, we can easily extend this to get a bound over all degree (exactly) $d$ polynomials. Now to allow for at most degree $d$ polynomials, we run the same bound on $d-1$ polynomials and so on until say $d/2$ beyond which we apply a trivial $q^{d/2}$ bound without losing much in the total error. The multiplication by $R(t)$ is permitted because the character is multiplicative. This also gives a way to extract from sources that can be encoded as polynomials and then the rich structure of polynomials can be put to good use.

We point out that polynomial AP sources are extremely structured additively as we saw above and falls in the general theme of this work. This is in sharp contrast to \textit{polynomial sources} which have been studied in \cite{dgw, BenG}. In such sources, the source outputs the value of the polynomial on a random input. However, here the source itself outputs polynomials.

\begin{comment}
\paragraph{Connection to Erdos Discrepancy Problem (EDP) over function fields}
The EDP is defined as follows. Does there exist $g:\Fq[t] \rightarrow \C$ and constant $C$ such that for all $d$, \[\l|\sum_{\deg(P)\leq d, monic P}g(P)\r| \leq C?\]
Over integers, as we mentioned in Section~\ref{sec:extrgap}\Anote{is this still there? else I can repeat here, or not}, we can find a function whose discrepancy grows logarithmically with $n$ \Anote{Gowers' blog}(instead of constant $C$). In the case of function fields, it is known that for large fields, there exists a $g$ satisfying the above property \Anote{Polymath cite}. However, in this work we prove that all non trivial multiplicative characters modulo $Q$ have small discrepancy (again, not constant $C$) even over small fields as long as $d$ is logarithmic in degree of $Q$ (logarithmic min-entropy). This is the best bound known so far. It is however well known that the Mobius function has low discrepancy as well. However, in the language of extractors, the Mobius function can extract only $1$ bit whereas by the XOR lemma, we can extract more bits from the character sum bound. This work makes a small step towards achieving a negative result of the EDP in the case of all finite fields.
\end{comment}

All implied constants in this section will depend on $q$.
Our main result in this section is the following.\\ \\  
\textbf{Theorem~\ref{THM:ff}.} There exists $C>0$ such that the following is true. Let $\Fq$ be a finite field with $q \geq C$. Let $Q$ be a monic irreducible polynomial of degree $n$. Then there exists an $\eps$-extractor $\ext:\F_{q^n} \rightarrow F_{q^m}$ for $d$-subideal sources where $d=\Omega(\log_q n)$ and $\eps=\l(\frac{1}{d/\log_q n}\r)^{O\l(d/\log_q n\r)}q^{m/2}$.

The theorem follows from a character sum bound which is the main technical lemma of this section and Lemma \ref{lem:multlem}. First let us define the character precisely. We shall be using multiplicative characters over finite fields. Let $\F_{q^n}$ be the finite field in consideration. We shall represent every field element by the canonical polynomial of degree $n-1$ modulo an irreducible polynomial $Q$ of degree $n$. If $Q \in \Fq[t]$ of degree $n$, $Q \neq 0$, then a \textit{(Dirichlet) 
 character} modulo $Q$ is a function $\chi: \Fq[t] \rightarrow \C$ satisfying the following conditions:
\begin{itemize}
 \item $\chi(f+gQ)=\chi(f)$ for any $f, g \in \Fq[t]$.
 \item $\chi(fg)=\chi(f)\chi(g)$ for any $,f,g \in \Fq[t]$.
 \item $\chi(f) \neq 0$ if and only if $(f,Q)=1$.
\end{itemize}
If $Q$ is irreducible, then $\chi$ is simply a multiplicative character of $\F_{q^n}$.

\begin{lem}\label{lem:ff}There exists $C>0$ such that the following is true. Let $\Fq$ be a finite field with $q \geq C$. 
Let $Q$ be a monic irreducible polynomial of degree $n>0$ in $\Fq[t]$ and $\chi$ be a non-trivial character modulo $Q$. Then for any $d \geq 24 (\log_q n+1)$, we have
\[
\left| \sum_{\substack{\deg(f) = d,\\ f \textup{ monic} }} \chi(f) \right| = O_q \left( N(d, 24 (\log_q n+1)) \right)
\] 
Here $N(d, r)$ is the number of monic polynomials of degree $d$, all of whose irreducible factors have degree $\leq r$.
\end{lem}
The function $N(d,r)$ will be described in more detail shortly, but we remark that as $d/r \rightarrow \infty$, we have
\[
N(d,r) = O \l( q^d \left(d/r \right)^{-(1+o(1))d/r} \left(1 + \frac{d \log d}{r^2} \right)\r)
\]
In particular, the bound given by Lemma \ref{lem:ff} is nontrivial as $\frac{d}{\log n} \rightarrow \infty$.

The constant 24 in Lemma \ref{lem:ff} can certainly be improved. Also, the condition that $q$ is sufficiently large can probably be dropped if we establish more refined versions of Lemmas \ref{lem:n1} and \ref{lem:n2}, though we don't seek to do so. 

\subsection{Number theoretic preliminaries in $\Fq[t]$}

An important property we shall use about the polynomials over a finite field is the notion of a norm.
\begin{define}[Norm of polynomial]For a non-zero polynomial $f \in \Fq[t]$, the \textit{norm} $|f|$ of $f$ is defined to be $q^{\deg(f)}$. We also define $|0|=0$. \end{define}

We will introduce Dirichlet series in $\Fq[t]$, which can be found in \cite[Chapter 4]{rosen}. We shall drop the $\chi$ from the arguments of all the functions below for notational brevity.
Suppose $Q \neq 0$ (not necessarily irreducible) and $\chi$ is a character modulo $Q$. The Dirichlet series corresponding to $\chi$, is defined by
\begin{equation}
 L(s)=\sum_{f \textup{ monic}} \frac{\chi(f)}{|f|^s}.
\end{equation}
where $s$ is any complex number.
It can be easily shown that $L(s)$ is convergent absolutely when $\textup{Re}(s)>1$.
In the case $Q=1$ and $\chi$ being the trivial character, we have the analog of Riemann's zeta function
\[
 \zeta(s)=\sum_{f \textup{ monic}} \frac{1}{|f|^s}
\]
 Since, we will be interested in character sums over monic polynomials, put
\begin{equation}
 A(m)= \sum_{\substack{\deg(f)=m,\\ f \textup{ monic} }} \chi(f).
\end{equation}

We will soon see that $A(m)$ vanishes whenever $m \geq \deg Q$. The challenge is to make the sum very small for small $m$. Think of $m$ (or $m \log q$) as the min-entropy of the source.
Now we have a succinct way to write the Dirichlet series.
\[ L(s)= \sum_{m=0}^{\infty} A(m) q^{-ms}\]
when $\textup{Re}(s)>1$. 

Next, we need another representation of the Dirichlet series. Here and throughout this section, $P$ stands for a monic, irreducible polynomial in $\Fq[t]$. 
\begin{define}[Euler decomposition]When $\textup{Re}(s)>1$, we have an Euler product decomposition
\[
 L(s)=\prod_{P} \left( 1 - \frac{\chi(P)}{|P|^s} \right)^{-1}\]
\end{define}

We shall make another notational simplification now. It is more convenient to work with the following variant of $L(s)$. Put
\begin{equation}
 \calL(z)= \sum_{m=0}^{\infty} A(m) z^{m}.
\end{equation}
Since $A(m)=0$ whenever $m\geq n$, $\calL(z)$ is a polynomial and in particular is an entire function. Clearly $L(s)=\calL(q^{-s})$ for any $\textup{Re}(s)>1$. From the Euler product formula, we have
\begin{equation} \label{eq:euler2}
 \calL(z)=\prod_{P} \left( 1 - \chi(P) z^{\deg(P)} \right)^{-1}
\end{equation}
whenever $|z|<1/q$. 

\begin{comment}It follows immediately that $\calL(z,\chi)$ is a polynomial of degree at most $n-1$. Consequently, $L(s,\chi)$ can be analytically continued to an entire function on 
$\mathbb{C}$. 
Clearly $\calL(z, \chi)$ can be written as
\begin{equation} \label{eq:zeroes}
 \calL(z, \chi) = \prod_{i=1}^{n-1} \left( 1 - \alpha_i (\chi) z\right)
\end{equation}
for some complex numbers $\alpha_i(\chi)$. The \textit{Generalized Riemann Hypothesis} for function fields, proved by Weil (for a proof, see \cite[Appendix]{rosen}), 
implies that for all $i$, $|\alpha_i|=\sqrt{q}$. 
\end{comment}

We now state the \textit{Generalized Riemann Hypothesis} for function fields which was proved by Weil in 1948 (for a proof, see \cite[Appendix]{rosen}).
%\begin{thm}\label{thm:riemann}Let $\calL$ be defined as above. If $\calL(z) = 0$, then $|z| = q^{-1/2}$.\end{thm}

%Another formulation of this theorem that we shall use is the following.
\begin{thm}\label{thm:riemann}Let $\calL$ be defined as above. Then, \[\calL(z) = \prod_{i=1}^{n-1} \left( 1 - \alpha_i z\right)\]
for some complex numbers $\alpha_i$ such that $|\alpha_i|=\sqrt{q}$.\end{thm}

Note that this implies $\calL(z) \neq 0$ when $|z| < q^{-1/2}$. 

The final quantity we need is the \textit{von Mangoldt function}.
\begin{define}[von Mangoldt function $\Lambda(f)$]For $f \in \Fq[t]$, if $f=P^k$, where $P$ is a monic irreducible polynomial and $k \in \Z^{+}$, 
then we define $\Lambda(f)=\deg(P)$. We define $\Lambda(f)= 0$ for all other $f$ (thus $\Lambda(f)$ is necessarily 0 if $f$ is not monic). 
\end{define}


\subsection{Basic facts and claims}
Let us prove some simple claims to get more familiar with the above quantities. We point out that this subsection is not novel and has been presented merely as a warmup for our main proof. The claims will be used crucially in the analysis. All the proofs have been included in the Appendix.


We first obtain a closed form expression for the $\zeta$ function. Recall that \[\zeta(s)=\sum_{f \textup{ monic}} \frac{1}{|f|^s}\]
\begin{claim} \label{clm:zeta}$\zeta(s) =\frac{1}{1-q^{1-s}}$
whenever $\textup{Re}(s)>1$.
\end{claim}


The next claim shows that the character sums $A(m)$ vanish when $m$ is large. More formally, we have the following.
\begin{claim}\label{clm:fullsum}Let $\deg Q=n>0$ and $\chi$ be non-trivial multiplicative character modulo $Q$. Then 
 $A(m)=0$ whenever $m \geq n$.
\end{claim}


The next claim is on the Euler decomposition. Using that we have an alternate expression for $\log \calL(z)$.
\begin{claim}\label{clm:euler}Let $|z|<1/q$. Then,
\[\log \calL(z) = \sum_{f \textup{ monic}} \frac{\Lambda(f) \chi(f)}{\deg(f)} z^{\deg(f)}\]
\end{claim}



Finally, we will need the following formula, known as Perron's formula.
\begin{lem}[Perron's formula, {\cite[Chapter 17]{davenport}}] \label{lem:perron} Let $c>0$. Then for any $y>0$, we have
\begin{enumerate} 
 \item 
\[  \frac{1}{ 2 \pi i} \int_{c-i \infty}^{c+i \infty} \frac{y^s}{s} ds = \begin{cases}
0, & \textup{ if } 0<y<1 \\
1, & \textup{ if } y>1.
\end{cases}
\]
\item If $T>0$, then
\[ \frac{1}{ 2 \pi i} \int_{c-i T}^{c+i T} \frac{y^s}{s} ds =
O \left( y^c \min \left( 1, \frac{1}{T | \log y|}\right) \right) +   
\begin{cases}
0, & \textup{ if } 0<y<1 \\
1, & \textup{ if } y>1.
\end{cases}
\]
\end{enumerate}

\end{lem}


\subsection{Smooth polynomials} \label{sec:smooth}
We shall also use the notion of smooth polynomials in our proof. Given an integer $m \geq 1$, we say a polynomial $f \in \Fq[t]$ is $m$\textit{-smooth} if all of its irreducible factors have degree $\leq m$. 
Let us denote by $\calS(m)$ the set of all monic $m$-smooth polynomials. 

Given integers $n \geq m \geq 1$, let us denote by $\calP(n,m)$ the set of all monic $m$-smooth polynomials $f$ such that $\deg(f)$ is exactly $n$. Also, let us denote by $\calS(n,m)$ the set of all monic $m$-smooth polynomials $f$ such that $\deg(f)$ is at most $n$. Let us put $N(n,m)=|\calP(n,m)|$. 

\begin{comment}
The function $N(n,m)$ is closely related to the \textit{Dickman function}. Recall that the Dickman function $\rho(u)$ is the unique continuous function satisfying 
\[
\rho(u) = \frac{1}{u} \int_{u-1}^u \rho(t) dt
\]
for all $u>1$, with initial condition $\rho(u)=1$ for $0 \leq u \leq 1$. The function $\rho(u)$ decays to 0 extremely rapidly as $u \rightarrow \infty$. More precisely, we have
\[
\rho(u) = u^{-u(1+o(1))} \qquad \textup{as} \, u \rightarrow \infty.
\]

Regarding $N(n,m)$, we have
\begin{thm}[Manstavi\v{c}ius \cite{mansta}]
For any $1 \leq m \leq n$, we have
\[
N(n,m) = q^n \rho \left(\frac{n}{m}\right) \left( 1 + O \left( \frac{n \log n}{m^2} \right) \right)
\]
\end{thm}
In particular, we have $N(n,m) \sim q^n \rho(n/m)$ as $n \rightarrow \infty$ and $\frac{m}{\sqrt{n \log n}} \rightarrow \infty$.
\end{comment}
%\Anote{check range of m. since only large m used, 1+o(1) term needed}
The following is a consequence of \cite[Theorem 1.3]{sound}.
\begin{lem}\label{lem:n1}
There exists an absolute constant $c$ such that for any $1 \leq m \leq n$, we have
\[
N(n-1,m) \leq \frac{cn^{1/m}}{q} N(n,m).
\]
Consequently, for any $m \leq t\leq n$, we have
\[
N(t,m) \leq \left(\frac{cn^{1/m}}{q}\right)^{n-t} N(n,m).
\]
\end{lem}

To gain some intuition for the above, observe that if $f \in \calP(n-1,m)$, then for every $a \in \Fq$, $(x-a)f \in \calP(n,m)$. Now assuming no over counting, this would mean that $N(n,m) \geq q N(n-1,m)$. The above lemma says that this is not far from the correct estimate.

%\Hnote{This should be true, and is an exact analog of Granville and Soundararajan's Proposition 3.5. Soundararajan's \cite[Theorem 1.3]{sound} looks very similar to this.}
Using the above, we prove the following straightforward lemma.
\begin{lem}\label{lem:n2}
Assume that $q$ is sufficiently large, say $q \geq (2c)^3$. Let $r \leq n$, and assume that $cd^{1/r} q^{1/r-1/2} <1/2$. Let $\kappa=1/2+1/r$. Then we have
\[
\sum_{f \in \calS(n,r)} q^{-\kappa \deg(f)} \leq 2 N(n,r) q^{-n\kappa}
\]
\end{lem}
\begin{proof}
Note that under the assumption on $r$, $c n^{1/r} q^{\kappa-1} < 1/ 2$.
\begin{eqnarray*}
\sum_{f \in \calS(n,r)} q^{-\kappa \deg(f)} &=& \sum_{i=r}^{n} q^{-\kappa i} N(i,r) \\
&=& \sum_{i=r}^{n} q^{-\kappa i} \left(\frac{cn^{1/r}}{q}\right)^{n-i} N(n,r) \\
&=& N(n,r) \left(\frac{cn^{1/r}}{q}\right)^{n} \sum_{i=r}^{n} \left( cn^{1/r}q^{\kappa -1} \right)^{-i} \\
&\leq& 2 N(n,r) \left(\frac{cn^{1/r}}{q}\right)^{n} \left( cn^{1/r}q^{\kappa -1} \right)^{-n} \\
&=& 2 N(n,r) q^{-n\kappa}
\end{eqnarray*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:ff}} \label{sec:ffproof}

We will only present the high level idea of the proof. Once the right quantities have been introduced, the proof is similar to \cite{gs} and uses standard tools of contour integrals. We shall however rely on a key lemma (Lemma~\ref{lem:bound3}) for our proof which we prove later. 

\begin{proof}[Proof of Lemma \ref{lem:ff}]
The idea of the proof is to approximate $A(d)$ by 
$A(d, r)$ for $r$ small. Here $A(d, r)$ is the \textit{smooth sum}
\[
A(d, r) = \sum_{f \in \calP(d,r)} \chi(f).
\]
This idea was used by Montgomery-Vaughan \cite{mv} and later by Granville-Soundararajan \cite{gs} in the context of integers. We use the idea to analyse character sums over polynomials. More precisely, we will obtain the estimate
 \[A(d)-A(d,r)=O \left( N(d,r) \exp \left( C n^4 c^r  q^{-r/2} \right) \right) \]
for some constant $C$. We can bound $A(d, r)$ trivially by $N(d,r)$. By making a judicious choice of $r$, this gives a bound on $A(d)$. The details of the proof can be seen in the Appendix. In some places, our proof uses power series and Cauchy's integral formula instead of Dirichlet series and Perron's formula. 
As such, it is cleaner than the proof for the integers.
\end{proof}

\subsubsection{The key Lemma \ref{lem:bound2}}


We introduce a new function which is the right analog over polynomials of the corresponding function over integers and upper bound it. 
\[
\calL(z,r)=\calL(z) \prod_{\deg(P) \leq r} \left( 1-\chi(P)z^{\deg(P)} \right).\] 
Note that if $|z| <1/q$, then we have $\calL(z, r)= \prod_{\deg(P)>r} \left( 1-\chi(P) z^{\deg(P)} \right)^{-1}$. 

We have the following bound for $\calL(z,r)$.

\begin{lem}\label{lem:bound3} 
Suppose $r\in \Z^{+}$ $|z|=q^{-\sigma}, \sigma \geq 1/2 + 1/r$. Then 
\[
|\log \calL(z,r)| = O \left( n r^2 \right)
\]
\end{lem}



We need the following lemma which we prove later. The lemma is essentially proving that the partial sum up to degree $r$ polynomials is close to the infinite sum (Recall Claim~\ref{clm:euler}).
\begin{lem}\label{lem:bound2}
Let $1/2< \sigma_1 < \sigma \leq 1 $ and $r$ be a positive integer. 

Then for any $|z|=q^{-\sigma}$, we have
\[
\log \calL(z)-\sum_{ \deg(f) \leq r} \frac{\Lambda(f)\chi(f)}{\deg(f)} z^{\deg(f)} =   O \left( \frac{n q^{r(\sigma_1 - \sigma)}}{\sigma_1-1/2} \left( r - \log (\sigma - \sigma_1) \right) \right).
\]
\end{lem}
With the above lemma in place, the proof of Lemma \ref{lem:bound3} follows similar to \cite{gs}.
We include it in the appendix.

We now prove Lemma \ref{lem:bound2}.

\begin{figure}
\hspace*{4cm}\includegraphics[width=0.5\textwidth, height=90mm]{pic.pdf}\label{fig:zeta}
\caption{The contour integral of $g(w)=\log \calL(zq^{-w})\frac{x^w}{w}$}
\end{figure}
\begin{proof}[Proof of Lemma \ref{lem:bound2}]Let $\Psi(f)$ be the shorthand for $\frac{\Lambda(f) \chi(f)}{\deg(f)}$. We first begin with a proof overview. We shall refer to Figure~\ref{fig:zeta}. We shall first prove that $\log \calL(z)$ is the residue of $g(w)=\log \calL(zq^{-w})\frac{x^w}{w}$ in the rectangular contour. This follows from the Riemann hypothesis after some thought. Next, we shall show that the integral of $g(w)$ on the red segment is close to the partial summation $\sum_{deg(f) \leq r}\Psi(f)$. Next, we show that each of the integrals on the remaining blue segments are small. Then by the Cauchy integral formula, the residue is close to the partial summation which completes the proof. The proof involves bounding the number theoretic quantities defined before on the ring of polynomials.


In the following, $\sum_f$ will be a shorthand for $\sum_{f \textup{ monic}}$. 
Let $x=q^{r+1/2}$ and $c=1-\sigma+1/r$. Then for any $w$ with $\textup{Re}(w)=c$, we have $|zq^{-w}|<1/q$. By Claim~\ref{clm:euler}, we have
\begin{equation} 
 \log \calL(zq^{-w}) = \sum_{f} \Psi(f) z^{\deg(f)} q^{-w \deg(f)}.
\end{equation}
Therefore,
\begin{eqnarray*}
\frac{1}{2\pi i}\int_{c-ix}^{c+ix}\log \calL(zq^{-w}) \frac{x^w}{w}dw
&=&\frac{1}{2\pi i}\int_{c-ix}^{c+ix}\sum_{f}\frac{\Lambda(f)\chi(f)}{\deg(f)} z^{\deg(f)}q^{-w \deg f} \cdot \frac{x^w}{w}dw\\
&=&\sum_{f}\frac{\Lambda(f)\chi(f)}{\deg f} z^{\deg(f)} \cdot \frac{1}{2\pi i}\int_{c-ix}^{c+ix}\frac{(x/|f|)^w}{w}dw.
\end{eqnarray*}
Note that we appended an $x^w/w$ term to the integrand to separate out the low degree part from the high degree (the error term). The integral of $x^w/w$ almost vanishes when the degree is large. To see this, by Perron's formula (Lemma~\ref{lem:perron}), the left side can be rewritten as
\begin{eqnarray}
& & \sum_{\deg(f) \leq r} \frac{\Lambda(f)\chi(f)}{ \deg(f)} z^{\deg(f)} + O \left( \sum_{f}\frac{\Lambda(f)}{ \deg(f)} |z|^{\deg(f)} \cdot 
\frac{ \left( \frac{x}{|f|} \right)^c}{x \left| \log \frac{x}{|f|} \right|} \right) \nonumber \\
&=&\sum_{\deg(f) \leq r}\frac{\Lambda(f)\chi(f)}{\deg(f)} z^{\deg(f)}+ O \left( \sum_{f} |z|^{\deg(f)} \cdot \frac{\left( \frac{x}{|f|} \right)^c}{x \left| \log \frac{x}{|f|} \right|}\right) \nonumber \\
&=&\sum_{\deg(f) \leq r}\frac{\Lambda(f)\chi(f)}{\deg(f)} z^{\deg(f)} +O\left(\frac{1}{x}\sum_{f}\frac{x^c}{|f|^{c+\sigma}\left| \log \frac{x}{|f|} \right|}\right). \label{eq:error1}
\end{eqnarray}
 We next bound the error term.
Note that by definition of $x$, 
$\left| \log \frac{x}{|f|} \right| \gg 1$ for all $f \neq 0$. Also, by Claim~\ref{clm:zeta}),
\begin{equation*}
\sum_{f \textup{ monic}}\frac{1}{|f|^{c+\sigma}} = \frac{1}{1-q^{1-(c+\sigma)}} = \frac{1}{1-q^{-1/r}} =O(1). 
\end{equation*}
Thus, we have 
\begin{equation} \label{eq:error2}
\frac{1}{x} \sum_{f \textup{ monic}} \frac{x^c}{|f|^{c+\sigma} \left| \log \frac{x}{|f|} \right| }  = O (x^{c-1}) = O\left( q^{-r \sigma} \right).
\end{equation}
It is important to observe that the error term was bounded because of the way $c$ was chosen (that is, $c+\sigma>1$).
Now, that the error term is bounded, we have only established that the integral of $\log \calL(zq^{-w})\frac{x^w}{w}$ on the vertical line $c-ix$ to $c+ix$ is close to our \emph{target} value (as in the statement of the lemma). To show that $\log \calL(z)$ is close to this value, we observe that this is the residue of the integrand inside a carefully chosen rectangle. It is clear that if the rectangle we choose only has $w=0$ as the only simple pole, and we can bound all the integrals along the four sides, then we bound the residue. See Figure~\ref{fig:zeta}. Consider the rectangle whose vertices are $c-ix, c+ix, \sigma_1-\sigma - ix$ and $\sigma_1-\sigma + ix$, and let
$g(w)=\log \calL(zq^{-w})\frac{x^w}{w}$ to avoid notational clutter. By the Generalized Riemann Hypothesis (Theorem~\ref{thm:riemann}), we have $\calL(zq^{-w}) \neq 0$ whenever $\sigma+w>1/2$. Notice that this is indeed the case everywhere in the rectangle described above. Therefore, $g(w)$ has a simple pole at $w=0$ with residue $\log \calL(z)$. 
Thus, we have
\begin{sloppy}
\begin{equation}
\frac{1}{2\pi i}\int_{c-ix}^{c+ix} g(w)dw =\log \calL(z) + \frac{1}{2\pi i}\int_{c-ix}^{\sigma_1-\sigma-ix}g(w)dw+ \frac{1}{2\pi i} \int_{\sigma_1-\sigma-ix}^{\sigma_1-\sigma+ix}g(w)dw + 
\frac{1}{2\pi i} \int_{\sigma_1-\sigma+ix}^{c+ix}g(w)dw.
\end{equation}
\end{sloppy}

Next, we shall need the following claim on the maximum value of the integrand, thus letting us loosely bound some of the integrals above.
We start with the following bound on $\log \calL(z,\chi)$ when $|z| < q^{-1/2}$. The bound will be useful only on points with $z<<q^{-1/2}$. We present a more elementary proof for the following (compared to \cite{gs} which appeals to the Borel-Caratheodory theorem instead).
\begin{claim}\label{clm:bound1}
Suppose $|z|=q^{-\sigma}$ where $\sigma >1/2$. Then we have 
\[\log \calL(z) = O \left( \frac{n}{\sigma-1/2} \right)\]
\end{claim}
We present the proof shortly.
We now use Lemma \ref{clm:bound1} to bound the right hand side. Observe that the second integral is over a line of arbitrarily large length. Therefore, we cannot simply pull out the maximum integrand value and multiply by the length of the line. However, we can do so in the first and third integral as the length is bounded and the integrand can bounded by Lemma~\ref{clm:bound1}. For the second integral we pull out a certain part of the integrand and then integrate. The second integral is therefore
\[
O\l(  \frac{nx^{\sigma_1 - \sigma}}{\sigma_1 - 1/2}   \int_{0}^{x} \frac{ds}{\sigma - \sigma_1 + is}\r) =O\l( \frac{n q^{r(\sigma_1 - \sigma)}}{\sigma_1 - 1/2} 
\left( r - \log (\sigma - \sigma_1) \right)  \r)
\]
The first and third integrals are
\[
 O\l( \frac{n}{\sigma_1 - 1/2} (c-\sigma_1 + \sigma) x^{c-1} \r) = O \l( \frac{n}{\sigma_1 - 1/2} q^{-r\sigma} \left(1 + 1/r - \sigma_1 \right)\r)
\]
Therefore,  
\begin{equation} \label{eq:error3}
\frac{1}{2\pi i}\int_{c-ix}^{c+ix} g(w)dw =\log \calL(z) + O \left( \frac{n q^{r(\sigma_1 - \sigma)}}{\sigma_1-1/2} \left( r - \log (\sigma - \sigma_1) \right) \right).
\end{equation}
By combining (\ref{eq:error1}), (\ref{eq:error2}), (\ref{eq:error3}) we have the desired estimate.
\end{proof}

%\vspace{10mm}
\begin{proof}[Proof of Claim~\ref{clm:bound1}]
By Theorem~\ref{thm:riemann} (and noticing that $\textup{Re}(1-\alpha_i z) >0$ for any $i=1,\ldots, n-1$), we have
\[
\log \calL(z) = \sum_{i=1}^{n-1} \log (1 - \alpha_i z).
\]
where each $|\alpha_i|=q^{1/2}$.
Thus it suffices to show that for each $i=1, \ldots, n-1$, we have
\[
 \log (1 - \alpha_i z) = O \left(\frac{1}{\sigma-1/2}\right).
\]
\begin{eqnarray*}
 \left| \log (1 - \alpha_i z) \right| &=& \left| \sum_{k=1}^{\infty} \frac{(\alpha_i z)^k}{k} \right| 
 \leq \sum_{k=1}^{\infty} \frac{|\alpha_i z|^k}{k} \\
 &\leq&  \sum_{k=1}^{\infty} q^{k(1/2 - \sigma)} 
 \leq \frac{1}{1 - q^{1/2 - \sigma}} = O \left( \frac{1}{\sigma - 1/2} \right).
\end{eqnarray*}

\end{proof}




==> extrzpPGC.tex <==
\section{Extractors for r-GAPs in $Z_p$ under Paley graph conjecture}
We first state the conjecture below and then the main theorem of this section.


\begin{conjecture}[$PG(\de)$]Let $\chi$ be a multiplicative character of $\Z_p^*$. Let $S,T \subseteq \Z_p$ such that $|S|, |T| >p^{\de}$. Then there exists $\eps>0$ such that \[\l| \sum_{s \in S, t \in T}\chi(s+t)\r|<|S||T|/p^{\eps}\]
\end{conjecture}


We begin with the main theorem of this section.
\begin{thm}\label{thm:PG}Let $p$ be such that $p-1$ have no large prime factors. There exists an explicit efficient  $2p^{-\eps}2^{m/2}$-extractor $\ext:\Z_p \rightarrow \{0,1\}^m$, for $\l(p^{4\de /r},r\r)$-GAP sources under $PG(\de)$ where $\eps=\eps(\de)$.
\end{thm}
We first prove a statement about APs ($r=1$) and later a statement for $r>1$ and later use Lemma \ref{lem:multlem} to prove the main theorem .


\begin{lem}Given an $AP$ $X=\{b_0+ab_1: 0 \leq a <l\}$, for any $k$ such that $l>p^{2\de}$, there is $\eps>0$ such that we have \[\l|\E_{x \in X}\chi(x)\r|<1/p^{\eps}+1/p^{\de}\]
\end{lem}
\begin{proof}
Let $k$ be an arbitrary integer and $l=kd$ such that $d>p^{\de}$. Remove this assumption later. 
For $-1 \leq i \leq k$, let \[S_i=\{ab_1: id \leq a <(i+1)d\}\] Also, let \[T=\{b_0+ab_1: 0 \leq a <d\}\] Now, $|S_i|, |T| = d>p^{\de}$ Thus, applying Conjecture $PG(\de)$, to each $S_i$ and $T$ pair, we get \[\l|\sum_{s \in S_i, t \in T}\chi(s+t)\r|<d^{2}/p^{\eps}\]
Consider $A=\sum_i \sum_{s \in S_i, t \in T}\chi(s+t)$. By the above, $|A|< (k+2)d^2/p^{\eps}$. Rewriting $A$ in another way, \[A=\sum_z m(z)\chi(z)\] where $m(z)$ is the number of times $\xi(z)$ occurs in $A$. Consider any $z=b_0+(xd+yb)$ where $0 \leq x \leq k-1$. Then $m(z)$ includes contribution from the following $2$ sets: $S_i$, $i \in \{x-1,x\}$.
Therefore, 
\begin{eqnarray*}
m(z)&= &\sum_{a \in \{d-y,y\}}a\\
&=&(d-y+y)\\
&=&d
\end{eqnarray*}
Now, if some $x_i=0$ or $x_i=k$, we won't have the above cancellation. We have $2(k-(k-1))d=2d$ such $z's$ each with $m(z) \leq d$.
Therefore, $|d\sum_{x \in X}\chi(x)|\leq kd^{2}/p^{\eps}+2d^{2}$. Setting $k=p^{\de}$ proves the theorem.

\end{proof}


\Anote{Can be generalized to more general sources}


\begin{lem}Given an $r-GAP$ $X=\{b_0+\sum_{i=1}^ra_ib_i: 0 \leq a_i <l\}$, for $r \geq 2$, $l>p^{\frac{\de}{\lfloor r/2 \rfloor}}$, we have \[\l|\E_{x \in X}\chi(x)\r|<1/p^{\eps}\]
\end{lem}
\begin{proof}
Since the GAP is proper, let $m=\lfloor r/2 \rfloor$. Let \[S=\{b_0+\sum_{i=1}^{m}a_ib_i: 0 \leq a_i <l\}\] and \[T=\{\sum_{i=m+1}^{r}a_ib_i: 0 \leq a_i <l\}\]
Then, since $|S|$, $|T|>p^{\de}$, by Conjecture $PG(\de)$, we have \[\l|\sum_{s \in S, t \in T}\chi(s+t)\r|=\l|\sum_{x \in X}\chi(x)\r|<1/p^{\eps}\]
This proves the theorem.
\end{proof}


Thus, combining the two lemmas above, we have the following.
\begin{lem}Given an $r-GAP$ $X=\{b_0+\sum_{i=1}^ra_ib_i: 0 \leq a_i <l\}$, for $r \geq 1$, $l>p^{\frac{4\de}{r}}$, we have \[|\E_{x \in X}\chi(x)|<2/p^{\eps}\]
\end{lem}

The proof of the main theorem now follows using the above lemma and the XOR lemma (Lemma \ref{lem:addlem}) and the efficiency of the extractor follows from the fact that the discrete logarithm in $\Z_p$ is efficiently computable if $p-1$ is smooth.


==> tobeadded.tex <==
\subsection{Extractors from character sum bounds}
We now prove a generalization of the XOR lemma on $\Z_N$ under a relaxed requirement on the character sums as made precise below. We note that not all the statements are specific to $\Z_N$. However, we stick to it for simplicity.
Throughout, let $N=\prod_{i=1}^nq_i$ where each distinct $q_i \geq p$ for some prime $p$. Let $\Z_N^*$ denote the units of $(\Z_N,*)$.
We state our main lemma below. The proof will be similar to that in \cite{Rao} but will require a more careful analysis.
\begin{lem}\label{lem:charsumzn}
\end{lem}

Before we prove our lemma, we need the following.

\begin{clm}\label{clm:cs}$\sum_{x \in \Z_N}|f(x)| \leq N^{3/2}\max_{\xi \in \Z_N}\l|\hat{f}(\xi)\r|$
\end{clm}

We will also need the following lemmas.
\begin{lem}\label{lem:xor}Let $X$ be a distribution on $\Z_N$ with $|\E_{X}\psi(X)| \leq \eps$ for every $\psi \in \Z_N^*$. Let $U$ be the uniform distribution on $\Z_N$. Let $\sigma: \Z_N \rightarrow \Z_M$ be a function such that for every character $\phi \in \Z_M$, we have \[\sum_{\xi \notin \Z_N^*}\l|\widehat{\phi \circ \sigma}(\xi)\r| \leq \tau\]
Then, $|\sigma(X)-\sigma(U)|<\tau \eps \sqrt{M}$.
\end{lem}
\begin{proof}Let $\phi \in \Z_M$ be a non trivial character. Note that the hypothesis $|\E_{X}\psi(X)| \leq \eps$ is equivalent to $|\widehat{X-U}(\psi)| \leq \eps /N$ for $\psi \neq 0$.
Then,
\begin{eqnarray*}
&&\widehat{\sigma(X)-\sigma(U)}(\phi)\\
&=&1/M\l|\sum{x \in \Z_N}\phi \circ \sigma (x) (X-U)(x)\r|\\
&=&N/M\l|\sum{\xi \in \Z_N}\widehat{\phi \circ \sigma} (\xi) \widehat{X-U}(\xi)\r|\\
&=&N/M\l|\sum{\xi \in \Z_N^*}\widehat{\phi \circ \sigma} (\xi) \widehat{X-U}(\xi)\r|\\
&&+N/M\l|\sum{\xi \notin \Z_N^*}\widehat{\phi \circ \sigma} (\xi) \widehat{X-U}(\xi)\r|\\
&\leq  & \eps \log N/M+n/p \log N/M
\end{eqnarray*}
where the first term follows from Lemma \ref{lem:rao} and the assumption and the second term follows from Lemma \ref{lem:genrao} and the trivial bound of $1$ for the absolute value of any character.

Now, for the trivial character we have $\widehat{\sigma(X)-\sigma(U)}(\phi)=0$ since $X$ and $U$ are distributions.
Thus, the lemma follows by Claim \ref{clm:cs}.
\end{proof}


We first begin with some preliminaries on the Dirichlet $L$-series in $\Fq[t]$ followed by some claims on smooth polynomials.
